The Data Station: Combining Data, Compute, and Market Forces

This paper introduces Data Stations, a new data architecture that we are designing to tackle some of the most challenging data problems that we face today: access to sensitive data; data discovery and integration; and governance and compliance. Data Stations depart from modern data lakes in that both data and derived data products, such as machine learning models, are sealed and cannot be directly seen, accessed, or downloaded by anyone. Data Stations do not deliver data to users; instead, users bring questions to data. This inversion of the usual relationship between data and compute mitigates many of the security risks that are otherwise associated with sharing and working with sensitive data. Data Stations are designed following the principle that many data problems require human involvement, and that incentives are the key to obtaining such involvement. To that end, Data Stations implement market designs to create, manage, and coordinate the use of incentives. We explain the motivation for this new kind of platform and its design.

==> sections/conclusion.tex <==
\section{Discussion}
\label{sec:conclusion}

Data Stations are a new way of sharing data, models, and derived
data products. They emphasize logical data centralization and mitigation of
problems at their root, as opposed to data federation scenarios. This design
simplifies the management of sensitive data at the cost of introducing
challenges related to the data-compute inversion. Those challenges are tackled via
data-unaware task capsules.


